SVP-CF: Selection via Proxy for Collaborative Filtering Data

We study the practical consequences of dataset sampling strategies on the performance of recommendation algorithms. Recommender systems are generally trained and evaluated on samples of larger datasets. Samples are often taken in a naive or ad-hoc fashion: e.g. by sampling a dataset randomly or by selecting users or items with many interactions. As we demonstrate, commonly-used data sampling schemes can have significant consequences on algorithm performance -- masking performance deficiencies in algorithms or altering the relative performance of algorithms, as compared to models trained on the complete dataset. Following this observation, this paper makes the following main contributions: (1) characterizing the effect of sampling on algorithm performance, in terms of algorithm and dataset characteristics (e.g. sparsity characteristics, sequential dynamics, etc.); and (2) designing SVP-CF, which is a data-specific sampling strategy, that aims to preserve the relative performance of models after sampling, and is especially suited to long-tail interaction data. Detailed experiments show that SVP-CF is more accurate than commonly used sampling schemes in retaining the relative ranking of different recommendation algorithms.

==> oracle_results.tex <==
\begin{table}[!ht]
    \begin{small} % normalsize, small, footnotesize
    \begin{center}
        \begin{tabular}{c c | c c c}
            \toprule
            $\mathcal{E}$ & $\Phi$ & \textbf{MSE} & \textbf{P@1} \\ \midrule
            
            \multicolumn{2}{c|}{Random} & 0.2336 & 25.2 \\ 
            \multicolumn{2}{c|}{User sampling \emph{w/} Bias-only SVP-CF-Prop} & -- & 30.6 \\ \midrule
            
            Handcrafted & Least squares & 0.1866 & 31.7 \\
            '' & XGBoost regression & 0.1163 & 43.9 \\
            '' & \oracle-regression & \underline{0.1008} & 51.2 \\ 
            '' & \oracle-ranking    & -- & 51.2 \\ \midrule
            
            GCN & Least squares & 0.1838 & 39.1 \\
            '' & XGBoost regression & 0.1231 & 43.9 \\
            '' & \oracle-regression & 0.1293 & 48.8 \\ 
            '' & \oracle-ranking    & -- & \underline{53.7} \\ \bottomrule
        \end{tabular}
    \end{center}
    \end{small}
    % \vspace{3.1mm}
    \caption{Results for predicting the best sampling scheme for a particular dataset over a germane metric. The MSE-value next to randomly choosing the sampling scheme represents the variance of the test-set. Best values are \underline{underlined}.}
    \label{oracle_results}
    % \vspace{-6mm} %Put here to reduce too much white space after your table
\end{table}
